Exploiting Contextual Information with Deep Neural Networks

Context matters! Nevertheless, there has not been much research in exploiting contextual information in deep neural networks. For most part, the entire usage of contextual information has been limited to recurrent neural networks. Attention models and capsule networks are two recent ways of introducing contextual information in non-recurrent models, however both of these algorithms have been developed after this work has started. In this thesis, we show that contextual information can be exploited in 2 fundamentally different ways: implicitly and explicitly. In the DeepScore project, where the usage of context is very important for the recognition of many tiny objects, we show that by carefully crafting convolutional architectures, we can achieve state-of-the-art results, while also being able to implicitly correctly distinguish between objects which are virtually identical, but have different meanings based on their surrounding. In parallel, we show that by explicitly designing algorithms (motivated from graph theory and game theory) that take into considerations the entire structure of the dataset, we can achieve state-of-the-art results in different topics like semi-supervised learning and similarity learning. To the best of our knowledge, we are the first to integrate graph-theoretical modules, carefully crafted for the problem of similarity learning and that are designed to consider contextual information, not only outperforming the other models, but also gaining a speed improvement while using a smaller number of parameters.

==> Thesis2.tex <==
\setstretch{1.3}  % It is better to have smaller font and larger line spacing than the other way round

% Define the page headers using the FancyHdr package and set up for one-sided printing
\fancyhead{}  % Clears all page headers and footers
\rhead{\thepage}  % Sets the right side header to show the page number
\lhead{}  % Clears the left side page header

\pagestyle{fancy}  % Finally, use the "fancy" page style to implement the FancyHdr headers

%% ----------------------------------------------------------------


%% ----------------------------------------------------------------
% The "Funny Quote Page"
\pagestyle{empty}  % No headers or footers for the following pages

\null\vfill
% Now comes the "Funny Quote", written in italics
\textit{Dedicated to my father, Sejdi Elezi}

\vfill\vfill\vfill\vfill\vfill\vfill\null
\clearpage  % Funny Quote page ended, start a new page
%% ----------------------------------------------------------------

% The Abstract Page
\addtotoc{Abstract}  % Add the "Abstract" page entry to the Contents

\abstract{Context matters! Nevertheless, there has not been much research in exploiting contextual information in deep neural networks. For most part, the entire usage of contextual information has been limited to recurrent neural networks. Attention models and capsule networks are two recent ways of introducing contextual information in non-recurrent models, however both of these algorithms have been developed after this work has started.

In this thesis, we show that contextual information can be exploited in $2$ fundamentally different ways: implicitly and explicitly. In the DeepScore project, where the usage of context is very important for the recognition of many tiny objects, we show that by carefully crafting convolutional architectures, we can achieve state-of-the-art results, while also being able to implicitly correctly distinguish between objects which are virtually identical, but have different meanings based on their surrounding. In parallel, we show that by explicitly designing algorithms (motivated from graph theory and game theory) that take into considerations the entire structure of the dataset, we can achieve state-of-the-art results in different topics like semi-supervised learning and similarity learning. 

To the best of our knowledge, we are the first to integrate graph-theoretical modules, carefully crafted for the problem of similarity learning and that are designed to consider contextual information, not only outperforming the other models, but also gaining a speed improvement while using a smaller number of parameters.
}

\clearpage  % Abstract ended, start a new page
%% ----------------------------------------------------------------

\setstretch{1.3}  % Reset the line-spacing to 1.3 for body text (if it has changed)

% The Acknowledgements page, for thanking everyone
\acknowledgements{
\addtocontents{toc}{\vspace{1em}}  % Add a gap in the Contents, for aesthetics
 I would like to thank my family, for being the most important part of my life. My late father Sejdi, who always wanted me to get a Ph.D. degree but whom will never see me getting it, my mother Kymete, my brothers Mentor, Armend and Petrit and my sister Merita. I would like to thank my sisters-in-law Alida and Ibe, and my nephews and nieces (Dian, Rina, Lejla, Anna, Samuel and the little Joel). I love you all!

I would like to give my deepest gratitude to my supervisor, professor Marcello Pelillo for pushing me to start a Ph.D. degree in the first place, and for advising me during the entire course of it. I believe that his invaluable advice has helped me become a better researcher, and see things in a different way. I would like to thank my friends and colleagues at Ca' Foscari University of Venice for helping me during the Ph.D. Thanks Ale, Marco, Leulee, Joshua, Mauro, Mara, Martina, Alvise and Stefano. Special thanks to Seba, whom was my primary collaborator during the entire Ph.D., and with whom I spent endless time (be it on Venice or Munich) discussing, coding, debugging and writing papers during the deadline sessions. I would like to thank Nicolla Miotello for being always helpful in all the administrative issues I had during the doctorate. I would like to thank the external reviewers, professor Marco Gori and professor Friedhelm Schwenker for giving valuable feedback on improving the thesis.

I spent a great year at Zurich University of Applied Sciences, being advised from professor Thilo Stadelmann. Thanks Thilo for having me there, and for helping me not only in the projects I was working on, but for giving me unconditional support and for being a great co-supervisor during the entire duration of my Ph.D. Thanks Thilo for volunteering to read an advanced draft of the thesis, and for giving me detailed feedback on how to improve it. I would like to thank Lukas with whom I did most of the work in DeepScore project while at ZHAW. I was lucky to have Lukas as my primary collaborator at ZHAW, and I found working with him both rewarding and enjoyable. I will never forget the time spent with the other members of the group (Mohammad, Kathy, Ana, Jonas, Mario, Melanie, Frank, Kurt, Andy and Martin).

I consider the highlight of my Ph.D. the time I spent at the Technical University of Munich. I went there (together with Seba) to work with professor Laura Leal-Taix\'{e}, a young professor I had only met twice before. Little I knew that during the next $9$ months, Laura would became my awesome supervisor, my mentor, a great friend, and beat me in table tennis, kicker, singstar, uno, codenames and bowling (though I had the last laugh in the Game of Thrones prediction game, but she does not accept it)! I will always be \textbf{\#grateful} to Laura for the opportunity she gave me to spend that time in her lab, for helping me become a better researcher, and for giving me the best supervision a student can ask for. I would also like to thank Laura's minions for making me feel part of the group. Tim, Qunjie, Patrick, Guillem, Aljosa, Aysim and Sergio, thank you guys, you rock. Special thanks to Maxim, with whom I worked a lot in a project which is not part of the thesis, but which was the most enjoyable project I have ever worked. If this group doesn't make the next big thing in computer vision, we are done! :)

Last but not least, I would like to thank Jose Alvarez for mentoring me at NVIDIA Research at Santa Clara. Together with him (and in collaboration with Laura) we are exploring an exciting project that deals with the combination of semi-supervised learning and active learning. I would like to thank the other members of the group (Akshay, Francois and Maying). Go green team!


}
\clearpage  % End of the Acknowledgements
%% ----------------------------------------------------------------

\pagestyle{fancy}  %The page style headers have been "empty" all this time, now use the "fancy" headers as defined before to bring them back


%% ----------------------------------------------------------------
\lhead{\emph{Contents}}  % Set the left side page header to "Contents"
\tableofcontents  % Write out the Table of Contents

%% ----------------------------------------------------------------
\lhead{\emph{List of Figures}}  % Set the left side page header to "List if Figures"
\listoffigures  % Write out the List of Figures

%% ----------------------------------------------------------------
\lhead{\emph{List of Tables}}  % Set the left side page header to "List of Tables"
\listoftables  % Write out the List of Tables

%% ----------------------------------------------------------------
\setstretch{1.5}  % Set the line spacing to 1.5, this makes the following tables easier to read
\clearpage  % Start a new page

\mainmatter	  % Begin normal, numeric (1,2,3...) page numbering
\pagestyle{plain}  % Return the page headers back to the "fancy" style


%\input{Chapters/Introduction}

%\input{Chapters/Fundamentals.tex}

%\input{Chapters/LabelAugmentation.tex}

%\input{Chapters/GroupLoss.tex}

%\input{Chapters/DeepScores.tex}

%\input{Chapters/DWD.tex}

%\input{Chapters/Conclusions.tex}

\appendix
%\input{Appendices/Clustering.tex}



\addtocontents{toc}{\vspace{2em}}  % Add a gap in the Contents, for aesthetics
\backmatter

\label{Bibliography}
\lhead{\emph{Bibliography}} 
\bibliographystyle{apa}
\bibliography{Bibliography}  
